A Generalization of the ASR Search Algorithm to 2-Generator Quasi-Twisted Codes

One of the main goals of coding theory is to construct codes with best possible parameters and properties. A special class of codes called quasi-twisted (QT) codes is well-known to produce codes with good parameters. Most of the work on QT codes has been over the 1-generator case. In this work, we focus on 2-generator QT codes and generalize the ASR algorithm that has been very effective to produce new linear codes from 1-generator QT codes. Moreover, we also generalize a recent algorithm to test equivalence of cyclic codes to constacyclic codes. This algorithm makes the ASR search even more effective. As a result of implementing our algorithm, we have found 103 QT codes that are new among the class of QT codes. Additionally, most of these codes possess the following additional properties: a) they have the same parameters as best known linear codes, and b) many of the have additional desired properties such as being LCD and dual-containing. Further, we have also found a binary 2-generator QT code that is new (record breaking) among all binary linear codes and its extension yields another record breaking binary linear code.

==> Alt/LCD.tex <==
\makeatletter
\def\old@comma{,}
\catcode`\,=13
\def,{%
  \ifmmode%
    \old@comma\discretionary{}{}{}%
  \else%
    \old@comma%
  \fi%
}
\makeatother
{
\centering
\begin{longtable}{l|l|p{0.70\linewidth}}
$ [195,38,58]_2$ & $3$ & $[ 6135332413622, 5511163061413, 0760162305021, 41167113347, 1304422614561 ]$\\
$ [172,42,46]_2$ & $3$ & $[ 16305255301422, 12552443046071, 26367761131227, 56712075265061 ]$\\
$ [170,32,52]_2$ & $5$ & $[ 15017544142, 62327171172, 5656706772, 54766743242, 50452552233 ]$\\
$ [165,32,50]_2$ & $3$ & $[ 7451352027, 7530304175, 16125740433, 70670753002, 2255573462 ]$\\
$ [164,40,44]_2$ & $3$ & $[ 0711720165373, 4162676126303, 731245452506, 4301603434632 ]$\\
$ [160,32,48]_2$ & $104$ & $[ 00542672771, 35714512512, 6146475721, 05016172172 ]$\\
$ [156,36,44]_2$ & $11$ & $[ 377230104735, 441101605347, 135525223756, 034664137676 ]$\\
$ [153,43,38]_2$ & $727$ & $[ 03362056173102, 273542165074071, 507007322260431 ]$\\
$ [141,46,32]_2$ & $3$ & $[ 340604477037257, 5555546265363011, 1447675154362301 ]$\\
$ [138,44,32]_2$ & $5$ & $[ 047572717636601, 042465541137103, 34632557665736 ]$\\
$ [124,30,36]_2$ & $3$ & $[ 3023466614, 104135571, 6774200266, 4032715624 ]$\\
$ [122,60,20]_2$ & $3$ & $[ 5714214006357625062, 32647415367136476374 ]$\\
$ [120,32,32]_2$ & $104$ & $[ 3211420427, 0605045201, 45670476662 ]$\\
$ [117,38,28]_2$ & $3$ & $[ 0466644754451, 2436541252673, 5131112141731 ]$\\
$ [116,28,34]_2$ & $3$ & $[ 442732531, 253642371, 2645552751, 4024662711 ]$\\
$ [114,54,20]_2$ & $11$ & $[ 350273450337664702, 105500762001021221 ]$\\
$ [111,36,26]_2$ & $3$ & $[ 515231504461, 200230765236, 126716101403 ]$\\
$ [110,50,20]_2$ & $14$ & $[ 03233320732245542, 03670445051210042 ]$\\
$ [110,40,24]_2$ & $730471$ & $[ 03646446602231, 6062203646014 ]$\\
$ [108,48,20]_2$ & $101$ & $[ 3300216514056443, 7000312523564625 ]$\\
$ [108,32,28]_2$ & $12$ & $[ 74160521111, 45604632562, 40250112373 ]$\\
$ [105,34,26]_2$ & $3$ & $[ 742252523401, 314437023031, 070422111261 ]$\\
$ [105,30,28]_2$ & $14$ & $[ 5153333215, 1365535577, 6626560476 ]$\\
$ [105,29,28]_2$ & $771$ & $[ 6162561672, 6651775572, 1064436731 ]$\\
$ [105,24,32]_2$ & $7367$ & $[ 51556275, 51764767, 20643705 ]$\\
$ [104,24,32]_2$ & $5$ & $[ 43441155, 53243002, 51421571, 06170414 ]$\\
$ [102,32,26]_2$ & $5$ & $[ 23016441171, 5155572505, 3261443103 ]$\\
$ [100,40,20]_2$ & $1002$ & $[ 3367605450137, 2264022063455 ]$\\
$ [99,32,24]_2$ & $3$ & $[ 65725410163, 17752117321, 5251344657 ]$\\
$ [99,31,25]_2$ & $7$ & $[ 23543624601, 1403477176, 00560656631 ]$\\
$ [99,30,26]_2$ & $11$ & $[ 0677144753, 1370221122, 461726547 ]$\\
$ [99,21,32]_2$ & $57731$ & $[ 2433502, 5112553, 6660032 ]$\\
$ [94,46,16]_2$ & $3$ & $[ 17570216336424, 6073617230441121 ]$\\
$ [93,30,24]_2$ & $3$ & $[ 7475563176, 4415177161, 234165126 ]$\\
$ [90,26,24]_2$ & $52$ & $[ 531435171, 114350132, 353040702 ]$\\
$ [90,24,26]_2$ & $101$ & $[ 60122111, 60321712, 23436313 ]$\\
$ [88,20,28]_2$ & $5$ & $[ 3324751, 701554, 5053663, 4071362 ]$\\
$ [84,24,24]_2$ & $12$ & $[ 37211625, 33260411, 43757466 ]$\\
$ [84,18,28]_2$ & $11$ & $[ 234021, 320241, 060265, 172327 ]$\\
$ [82,20,26]_2$ & $70215061$ & $[ 7157701, 570521 ]$\\
$ [81,19,26]_2$ & $777$ & $[ 726367, 21155, 303002 ]$\\
$ [78,24,22]_2$ & $5$ & $[ 27512541, 02121473, 60544261 ]$\\
$ [70,28,16]_2$ & $102$ & $[ 324234467, 0654036141 ]$\\
$ [63,20,18]_2$ & $3$ & $[ 4312562, 4302502, 5233323 ]$\\
$ [63,13,24]_2$ & $575$ & $[ 04021, 5456, 67011 ]$\\
$ [62,30,12]_2$ & $3$ & $[ 3024406253, 4560604406 ]$\\
$ [60,16,20]_2$ & $12$ & $[ 724711, 50616, 334001 ]$\\
$ [58,28,12]_2$ & $3$ & $[ 4127557501, 402073244 ]$\\
$ [56,24,12]_2$ & $12$ & $[ 67163116, 53054674 ]$\\
$ [52,24,12]_2$ & $5$ & $[ 7360021, 5267555 ]$\\
$ [51,16,16]_2$ & $3$ & $[ 623251, 7054, 15702 ]$\\
$ [50,20,12]_2$ & $14$ & $[ 0150542, 3034521 ]$\\
$ [34,16,8]_2$ & $3$ & $[ 71404, 010461 ]$\\
\caption{New Linear Complementary Dual Codes}
\label{tab:my_label}
\end{longtable}
}


==> Alt/Sorth.tex <==
\begin{table}
    \centering
    \begin{tabular}{l|l|p{0.70\linewidth}}
        $ [213,35,68]_2$ & $7120103605521$ & $[ 111124074763, 432070306671, 774512423733
]$\\
$ [158,39,44]_2$ & $35441216370232$ & $[ 5172674573162, 1174545113363 ]$\\
$ [155,10,72]_2$ & $16502701$ & $[ 554, 4101, 57, 011, 7701 ]$\\
$ [140,16,56]_2$ & $5033712$ & $[ 605031, 630121, 253451, 376371 ]$\\
$ [126,11,56]_2$ & $5232$ & $[ 3761, 0012, 5523, 5302, 1202, 454 ]$\\
$ [120,18,44]_2$ & $52101$ & $[ 241454, 375415, 221446, 331264 ]$\\
$ [112,19,40]_2$ & $5021$ & $[ 373773, 5774151, 356755, 1433301 ]$\\
$ [112,12,48]_2$ & $124002$ & $[ 4705, 7007, 5277, 0453 ]$\\
$ [110,34,28]_2$ & $76653211$ & $[ 60526046436, 202251730361 ]$\\
$ [110,24,36]_2$ & $55500752743$ & $[ 57222225, 34412755 ]$\\
$ [110,20,4]_2$ & $376515033775$ & $[ 3515263, 3706541 ]$\\
$ [108,21,36]_2$ & $111$ & $[ 5620102, 4110132, 2126317, 1604673 ]$\\
$ [100,21,32]_2$ & $73$ & $[ 0321052, 4140743, 1474414, 5140361 ]$\\
$ [96,20,32]_2$ & $12$ & $[ 140153, 6631273, 5771431, 4224433 ]$\\
$ [96,19,32]_2$ & $55$ & $[ 7522251, 653453, 631473, 627777 ]$\\
$ [93,15,36]_2$ & $525412$ & $[ 73036, 34767, 46131 ]$\\
$ [92,11,40]_2$ & $73221$ & $[ 3072, 046, 6641, 4673 ]$\\
$ [92,11,40]_2$ & $73221$ & $[ 3072, 046, 6641, 4673 ]$\\
$ [90,9,40]_2$ & $3$ & $[ 111, 551, 534, 455, 015, 615, 375, 645, 07 ]$\\
$ [88,21,28]_2$ & $3$ & $[ 0407703, 2145355, 7260573, 021165 ]$\\
$ [84,19,28]_2$ & $7$ & $[ 766644, 751675, 3504451, 551303 ]$\\
$ [84,15,32]_2$ & $51153$ & $[ 05752, 63554, 64613 ]$\\
$ [84,14,32]_2$ & $102$ & $[ 12042, 57752, 42473, 06653 ]$\\
$ [80,17,28]_2$ & $71$ & $[ 401643, 651151, 232501, 614002 ]$\\
$ [80,14,32]_2$ & $341$ & $[ 25232, 7, 0424, 6411 ]$\\
$ [80,13,32]_2$ & $542$ & $[ 41121, 4374, 65241, 3205 ]$\\
$ [80,12,32]_2$ & $525$ & $[ 5233, 5531, 4743, 534 ]$\\
$ [78,26,20]_2$ & $70112$ & $[ 000061552, 033006061 ]$\\
$ [78,12,32]_2$ & $3625345231$ & $[ 4532, 2146 ]$\\
$ [75,20,24]_2$ & $14$ & $[ 0027423, 726242, 3710732 ]$\\
$ [70,31,16]_2$ & $53$ & $[ 0215201037, 17453360511 ]$\\
$ [70,31,16]_2$ & $53$ & $[ 0215201037, 17453360511 ]$\\
$ [69,22,20]_2$ & $3$ & $[ 12325661, 6003045, 10405 ]$\\
$ [66,20,20]_2$ & $5$ & $[ 3343631, 027677, 0516553 ]$\\
$ [64,13,24]_2$ & $71$ & $[ 50421, 2344, 4624, 17661 ]$\\
$ [62,25,16]_2$ & $131$ & $[ 516317651, 45156344 ]$\\
$ [60,17,20]_2$ & $71$ & $[ 222761, 753102, 52627 ]$\\
$ [54,12,20]_2$ & $101$ & $[ 5233, 1144, 1726 ]$\\
$ [46,12,16]_2$ & $5616$ & $[ 5733, 6557 ]$\\

    \end{tabular}
    \caption{New Self-Orthogonal Codes}
    \label{tab:my_label}
\end{table} 

==> Alt/SorthRev.tex <==

\begin{table}
    \centering
    \begin{tabular}{l|l|p{0.70\linewidth}}
        $ [86,15,32]_2$ & $7265566153$ & $[ 13137, 36214 ]$\\
$ [70,30,16]_2$ & $14$ & $[ 1367566016, 5714137543 ]$\\
$ [68,16,24]_2$ & $1052101$ & $[ 46104, 27027 ]$\\
$ [52,25,12]_2$ & $3$ & $[ 406264731, 13441301 ]$\\
    \end{tabular}
    \caption{New Self-Orthogonal and Reversible Codes}
    \label{tab:my_label}
\end{table}

==> Tables/Sorth.tex <==

 %\begin{comment}
\begin{table}
    \centering
    \caption{New QT Codes that are Self-Orthogonal}
    \begin{tabular}{l|l|p{0.70\linewidth}}
$[n,k,d]_q$ & $g$ & $[f_1,...,f_\ell]$\\
\hline&&\\
$ [213,35,68]_2$ & [$7120103605521] ,[123456899877968667887]$  & $[ 111124074763, 432070306671, 7745124237338888888888888888888888], [2132144411221,523879233974]
]$\\
$ [158,39,44]_2$ & $35441216370232$ & $[ 5172674573162, 1174545113363 ]$\\
$ [93,15,36]_2$ & $525412$ & $[ 73036, 34767, 46131 ]$\\
$ [70,31,16]_2$ & $53$ & $[ 0215201037, 17453360511 ]$\\
$ [69,22,20]_2$ & $3$ & $[ 12325661, 6003045, 10405 ]$\\
$ [66,20,20]_2$ & $5$ & $[ 3343631, 027677, 0516553 ]$\\
    \end{tabular}
    \label{tab:my_label}
\end{table}
 %\end{comment}

==> Tables/SorthRev.tex <==
\begin{comment}
\begin{table}{
    \centering
    \caption{New Binary QC Codes that are Self-Orthogonal and Reversible}
    
    \begin{tabular}{l|l|p{0.70\linewidth}}
$[n,k,d]_q$ & $g$ & $[f_1,...,f_\ell]$\\
\hline&&\\
$ [70,30,16]_2$ & $14$ & $[ 1367566016, 5714137543 ]$\\
$ [52,25,12]_2$ & $3$ & $[ 156307741, 752562251 ]$\\
    \end{tabular}
    \label{tab:my_label}
}
\end{table}
\end{comment}

==> Tables/record.tex <==



\begin{table}[H]
    \centering 
    \begin{tabular}{l|l|p{0.30\linewidth}}
$[n,k,d]_q$ & $g_1,g_2$ & $[f_1,...,f_\ell]$\\
\hline&&\\
$ [111,38,25]_2 $ & $[1],[1111111111111111111111111111111111111]$ & $[[0011111111100011001101111111000010011],[011110110111110011011010101100100111],[111110000100000010100010101110000101]],[[0],[1],[1]]$


    \end{tabular}
    \label{tab:my_label}
\end{table}


